Automatic Ply Partitioning for Laminar Composite Process Planning

This work introduces an automated ply partitioning strategy for large-scale laminar composite manufacturing. It specifically targets the problem of fabricating large plies from available spooled materials, while minimizing the adverse effects on part quality. The proposed method inserts fiber-aligned seams sequentially until each resulting sub-ply can be manufactured from available materials, while simultaneously enforcing constraints to avoid quality issues induced by the stacking of seams across multiple plies. Leveraging the developable nature of individual plies, the partitioning problem is cast as a sequence of one-dimensional piecewise linear optimization problems, thus allowing for efficient local optimization via linear programming. We experimentally demonstrate that coupling the local search with a greedy global search produces the same results as an exhaustive search. The resulting automated method provides an efficient and robust alternative to the existing trial-and-error approach, and can be readily integrated into state-of-the-art composite design workflows. In addition, this formulation enables the inclusion of common constraints regarding laminate thickness tolerance, sub-ply geometry, stay-out zones, material wastage, etc. The efficacy of the proposed method is demonstrated through its application to the surface of an airplane wing and to the body panels of an armored vehicle, each subject to various performance and manufacturing-related geometric constraints.

==> glossary.tex <==
\section{Terminology}

\textbf{ply} single layer or sheet of fiber-matrix material with prescribed composition and fiber orientation \\
\textbf{laminar composite} layered structure consisting of multiple bonded matrix-impregnated fiber plies \\
\textbf{sub-ply} portion of a ply bounded by two adjacent seams \\
\textbf{layup} specific arrangement and stacking sequence of layers or plies of different materials used in the construction of a composite structure \\
\textbf{tooling} the tools, equipment, and fixtures used in the manufacturing process

